The Continuous Rank Probability Score of a Generalized Beta-Prime Distribution and Some Special Cases

This working paper describes new results in derivations of the Continuous Ranked Probability Score of a generalized beta-prime distribution and several special cases, such as the Dagum distribution and Singh-Maddala distribution. Comparison with Monte Carlo estimates is also presented.

==> body.tex <==
\begin{proof}
    We will leverage the form of the CRPS given by Eq. \eqref{eq:crps_alternate}, allowing us to evaluate the rule in parts rather than through the integral form given by Eq. \textcolor{red}{the integral form of the rule}.
    
    The first term in Eq. \eqref{eq:crps_alternate} is the expected absolute deviation from the observation, given by 

    \begin{equation*}
        \Expect{\abs{X-y}}  = \int_{0}^y(y-x)f_X(x)\diffd x + \int_{y}^{\infty}(x-y)f_{X}(x)\diffd x
    \end{equation*}
    This equation can be split up into two integrals, one with integrand $yf_{X}(x)$ and one with integrand $xf_{X}(x)$. The former integration is 
    \begin{equation*}
        \int_{0}^y yf_X(x)\diffd x - \int_y^{\infty}yf_X(x)\diffd x = y(2F(y|\alpha,\beta,p,q)-1)
    \end{equation*}
    and the latter is given by
    \begin{align*}
        \int_y^{\infty}xf_X(x)\diffd x -\int_0^yxf_X(x)\diffd x = \mu -2\int_0^yxf_X(x)\diffd x        
    \end{align*}
    Since $X$ has a GBP distribution, we can write this integral as 

    \begin{align*}
        \int_0^yxf_X(x)\diffd x &= \frac{p}{B(\alpha,\beta)}\int_0^y \left(\frac{x}{q}\right)^{\alpha p} \frac{1}{\left(1+(x/q)^p\right)^{\alpha+\beta}}\diffd x \\
        &=q\frac{B(\alpha+p^{-1},\beta-p^{-1})}{B(\alpha,\beta)}F(y|\alpha+p^{-1},\beta-p^{-1},p,q)\\
        & = \mu F(y|\alpha+p^{-1},\beta-p^{-1},p,q)
    \end{align*}
    So, we have that 
    \begin{equation}\label{eq:crpsBP_expabsxminusy}
        \Expect{\abs{X-y}}  = y\left(2F(y|\alpha,\beta, p,q)-1\right)+ 
         \mu\left(1-2F\left(y|\alpha+\frac{1}{p},\beta-\frac{1}{p}, p,q\right)\right)
    \end{equation}
    giving us the first two terms of Eq. \eqref{eq:crps_BP}. 

    Now it remains to evaluate $ \Expect{X\left(2F(X)-1\right)}$. The last term in the expectation is $-\mu$, so we turn our attention to $\Expect{2XF(X)}$. By Fubini's Theorem we can write that 
    \begin{align*}
        \Expect{XF(X)} = \int_o^{\infty}xf_X(x)\int_0^x f_X(t)\diffd t\diffd x = \int_0^{\infty}f_X(t)\int_t^{\infty}xf_X(x)\diffd x \diffd t
    \end{align*}

    The inner integral is equal to $\mu - \int_0^txf_X(x)\diffd x$. Again given the PDF of the GBP distribution we can see that

    \begin{equation*}
        \int_0^txf_X(x)\diffd x = \mu F(t|\alpha+p^{-1},\beta-p^{-1},p,q)
    \end{equation*}
    so the inner integral is equal to $\mu(1-F(t|\alpha+p^{-1},\beta-p^{-1},p,q))$, and 
    \begin{align*}
         \Expect{XF(X)} = \mu\left(1-\int_0^{\infty}f_X(t)F(t|\alpha+p^{-1},\beta-p^{-1},p,q)\diffd t \right)
    \end{align*}

    Now, to proceed we need to write the CDF of the GBP distribution. Say that $Y\sim BP(\alpha,\beta)=GBP(\alpha,\beta, 1, 1)$, then let $X = qY^{1/p}$. Then $\Prob{X<x } = \Prob{Y < \left(\frac{x}{q}\right)^p} = I_{\frac{x^p}{x^p+q^p}}\left(\alpha,\beta\right)$ where $I_z(\alpha,\beta)$ is the regularized incomplete Beta function. Since $X\sim GBP(\alpha,\beta, p, q)$ this is the CDF of the distribution. 

    Now we have to consider properties of the regularized incomplete Beta function $I_z(a,b)$. From \cite[\href{https://dlmf.nist.gov/8.17E19}{Eq. (8.17.19)}]{NIST:DLMF} we can see that $I_z(a,b)$ satisfies the recurrence relation

    \begin{equation*}
       I_z(a,b) = I_z(a-1,b+1) - \frac{z^{a-1}(1-z)^b}{bB(a,b)}
    \end{equation*}
    and therefore that, since $p=1/N$,
    \begin{align}\label{eq:incompletebetafn_recurrence}
        I_z(\alpha+p^{-1},\beta-p^{-1}) = I_z(\alpha,\beta)-\sum_{n=1}^N\frac{z^{\alpha+n-1}(1-z)^{\beta-n}}{(\beta-n)B(\alpha+n,\beta-n)}
    \end{align}

    Now let $x=\frac{x^p}{x^p+q^p}$, and we can see that this can be written as a recurrence relation for $F(x|\alpha+p^{-1},\beta-p^{-1}, p,q)$ as 

    \begin{align}
        \label{eq:cdf_recurrence}
        F(x |\alpha+p^{-1},\beta-p^{-1},p,q) = F(x|\alpha,\beta,p,q)-\sum_{n=1}^N\frac{(x/q)^{p(\alpha+n-1)}}{(\beta-n)B(\alpha+n,\beta-n)(1+(x/q)^p)^{\alpha+\beta-1}}
    \end{align}
    Using Eq. \eqref{eq:cdf_recurrence}, we can split the integral $\int_{0}^{\infty}F(x|\alpha+p^{-1},\beta-p^{-1},p,q)f(x|\alpha,\beta,p,q)\diffd x$ into two parts. The first part is $\int_0^{\infty}F(x|\alpha ,\beta ,p,q)f(x|\alpha,\beta,p,q)\diffd x = \int_0^{\infty}F(x|\alpha ,\beta ,p,q)\diffd F(x|\alpha ,\beta ,p,q) =\frac{1}{2}$, and the second can be evaluated term by term. From the form of the sum in Eq. \eqref{eq:cdf_recurrence} we can see that for a single value of $n$

    \begin{align*}
        &\int_0^{\infty} \frac{(x/q)^{p(\alpha+n-1)}}{(1+(x/q)^p)^{\alpha+\beta-1} }f(x|\alpha,\beta, p,q)\diffd x
        = \frac{p}{qB(\alpha,\beta)}\int_0^{\infty}\frac{(x/q)^{p(2\alpha+n-1)-1}}{(1+(x/q)^p)^{2\alpha+2\beta-1}} \diffd x \\
        =& \frac{B(2\alpha+n-1,2\beta-n)}{B(\alpha,\beta)}
    \end{align*}
     by relating the integrand to the PDF of the $BP(2\alpha+n-1,2\beta-n,p,q)$ distribution. From this, we can finally see that 

     \begin{equation}
         \Expect{2XF(X)} = 2\mu\left(\frac{1}{2} - \frac{1}{B(\alpha,\beta)}\sum_{n=1}^N \frac{B(2\alpha+n-1,2\beta-n)}{(\beta-n)B(\alpha+n,\beta-n)}\right)  
     \end{equation}
     and therefore that 
     \begin{equation}
         \Expect{X(2F(X)-1)} =  - \frac{2\mu}{B(\alpha,\beta)}\sum_{n=1}^N \frac{B(2\alpha+n-1,2\beta-n)}{(\beta-n)B(\alpha+n,\beta-n)}  
     \end{equation}
     From this and Eq. \eqref{eq:crpsBP_expabsxminusy} we see that
     \begin{equation}
         \begin{split}
             \Expect{\abs{X-y}} - \Expect{X\left(2F(X)-1\right)}= y\left(2F(y|\alpha,\beta, p,q)-1\right)+\\
        \mu\left(1-2F\left(y|\alpha+\frac{1}{p},\beta-\frac{1}{p}, p,q\right)+\frac{2}{B(\alpha,\beta)}\sum_{n=1}^N \frac{1}{\beta-n}\frac{B(2\alpha+n-1,2\beta-n)}{B(\alpha+n,\beta-n)}\right)
         \end{split}
     \end{equation}
     as desired.
\end{proof}
